IoT-Based Preventive Mental Health Using Knowledge Graphs and Standards for Better Well-Being

Sustainable Development Goals (SDGs) give the UN a road map for development with Agenda 2030 as a target. SDG3 "Good Health and Well-Being" ensures healthy lives and promotes well-being for all ages. Digital technologies can support SDG3. Burnout and even depression could be reduced by encouraging better preventive health. Due to the lack of patient knowledge and focus to take care of their health, it is necessary to help patients before it is too late. New trends such as positive psychology and mindfulness are highly encouraged in the USA. Digital Twins (DTs) can help with the continuous monitoring of emotion using physiological signals (e.g., collected via wearables). DTs facilitate monitoring and provide constant health insight to improve quality of life and well-being with better personalization. Healthcare DTs challenges are standardizing data formats, communication protocols, and data exchange mechanisms. As an example, ISO has the ISO/IEC JTC 1/SC 41 Internet of Things (IoT) and DTs Working Group, with standards such as "ISO/IEC 21823-3:2021 IoT - Interoperability for IoT Systems - Part 3 Semantic interoperability", "ISO/IEC CD 30178 - IoT - Data format, value and coding". To achieve those data integration and knowledge challenges, we designed the Mental Health Knowledge Graph (ontology and dataset) to boost mental health. As an example, explicit knowledge is described such as chocolate contains magnesium which is recommended for depression. The Knowledge Graph (KG) acquires knowledge from ontology-based mental health projects classified within the LOV4IoT ontology catalog (Emotion, Depression, and Mental Health). Furthermore, the KG is mapped to standards when possible. Standards from ETSI SmartM2M can be used such as SAREF4EHAW to represent medical devices and sensors, but also ITU/WHO, ISO, W3C, NIST, and IEEE standards relevant to mental health can be considered.

==> Sections/Evaluation/EvaluationStressDataset.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Section:  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Future Work - Evaluation: Stress Dataset}
\label{section:evaluation}
% Philip Schmidt, Robert Bosch GmbH, Corporate Research, Germany, firstname.lastname '@' de.bosch.com
% Attila Reiss, Robert Bosch GmbH, Corporate Research, Germany, firstname.lastname '@' de.bosch.com

A future work could be the usage of the 
\textbf{WESAD (Wearable Stress and Affect Detection)} dataset\footnote{\url{https://ubicomp.eti.uni-siegen.de/home/datasets/icmi18/}} to evaluate the work. The WESAD dataset contains data from 15 subjects during a stress-affect lab study while wearing physiological and motion sensors \citep{schmidt2018introducing}.
Raw sensor data was recorded with two devices: a chest-worn device (RespiBAN) and a wrist-worn device (Empatica E4).
The RespiBAN device provides the following sensor data: electrocardiogram (ECG), electrodermal activity (EDA), electromyogram (EMG), respiration, body temperature, and three-axis acceleration. The Empatica E4 device provides the following sensor data: blood volume pulse (BVP, 64 Hz), electrodermal activity (EDA, 4 Hz), body temperature (4 Hz), and three-axis acceleration (32 Hz).
Three different affective states (neutral, stress, amusement) are considered.

As future work, if needed other mental health datasets could be found on the Linked Open Data Cloud or Kaggle.



% Reasoning
% and common machine learning methods (Decision Tree (DT), Random Forest (RF), AdaBoost (AB), Linear Discriminant Analysis (LDA) and k-nearest neighbour (kNN)).

% blood volume pulse (BVP), electrocardiogram (ECG), electrodermal activity (EDA), electromyogram (EMG), respiration (RESP), body temperature (TEMP), and threeaxis acceleration (ACC).

% These results should be interpreted with caution due to the limitations of WESAD, regarding the number of subjects and the lack of age and gender diversity.

% Nevertheless, since using the LOSO evaluation scheme, our results indicate that generalisation is possible.


% blood volume pulse, electrocardiogram, electrodermal activity, electromyogram, respiration, body temperature, and threeaxis acceleration.

% by containing three different affective states (neutral, stress, amusement).

% https://archive.ics.uci.edu/ml/datasets/WESAD+%28Wearable+Stress+and+Affect+Detection%29


% Picard et al. [19] published a dataset containing physiological data recorded from one person, who is subject to eight different emotional stimuli over 20 days.

==> Sections/RelatedWork/Memento_albraikan2019inharmony.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ottawa

% PhD thesis: inHarmony: A Digital Twin For Emotional Well-being \cite{albraikan2019inharmony}


% (Albraikan et al. 
\textbf{inHarmony \citep{albraikan2019inharmony}} is an Emotional Well-being Digital Twin applied to the workplace. It includes emotion detection, emotional biofeedback, and emotion-aware recommender systems. A usability study was carried out with 35 practitioners wearing the Empatica E4 sensor to acquire physiological signals.


% we collected sufficient physiological data from 18 subjects using five induced emotions (neutral, cheer, sad, erotic and horror) to investigate the performance of physiological responses toward emotion recognition in a user-independent scenario.
% obtained hundreds of records of physiological signals for each emotion.

% emotion-aware digital twin.
% emotion-regulation routine.

% real-time mobile biofeedback system that uses wearable sensors to depict five basic emotions and provides the user with emotional feedback.

% emotional digital twin, including emotion detection, emotional biofeedback, and emotion-aware recommender systems.


% inHarmony: Another usability study could be conducted with more participants.

% increasing productivity and efficiency, improving staff morale and reducing absenteeism).

% inHarmony to be reliable, comprehensive, trustworthy and useful, and easy to use.

% five emotions: neutral, happy, sad, erotic, and horror.
% emotion-aware biofeedback systems
% Real-time emotion recognition using physiological signals was used to access the recommendations.

% sensing how other people feel will improve empathy skills and power relationships.

% reading a group’s emotions to discern the cause of the feelings, the system can help an organization address the needs of individuals and improve its ability to gain trust and influence.

% WMD-DTW learned the dynamic nature of the emotion and the individual differences in the variability of emotional intensity over time without the need for group-based models.


% RQ1. For emotional well-being, to what extent does the system help 
% a) illustrate the proposed goals, requirements, methods and constraints?
% b) improve emotional well-being?
% RQ2. What are the usefulness and usability of the proposed inHarmony system for emotional well-being?

% emotion-aware systems through the notion of digital twins and LBFs.
% we develop an emotionaware biofeedback system.
% emotion recognition algorithm using physiological signals that can then enable the development of LBF systems
% personalized recommendations
% erceived usefulness and effectiveness of the digital twin system in the workplace.

% emotion recognition systems using physiological information, including physiological signal data acquisition, preprocessing, feature extraction, feature selection, and classification. We also discuss several existing LBF domains.

==> TODO/TODO.tex <==
TODO march 2024


% \todo[inline]{TODO: double-check mental health for all of those standardization bodies}

% \todo[inline]{TODO: picture health standards for all of those standardization bodies}

==> dump.tex <==
Large Language Models (LLMs) have found extensive applications in mental health. \cite{hua2024large} highlighted two categories of using LLMs: tuning-free prompting and instruction fine-tuning. In the tuning-free prompting category, several publicly available models include Replika, Task-Adaptive Tokenization, Diagnosis of Thought Prompting, and ChatCBPTSD. These are based on GPT-3, LLaMA, GPT-3.5/GPT-4, and GPT-3.5 respectively. Meanwhile, other models, like DSC, MindShift, Psy-LLM, LLM-Counselors, Chain of Empathy Prompting (all GPT-3.5 based), MindfulDiary (GPT-4 based), and Female Firearm Suicides (FLAN-UL2 based) are not publicly available. Additionally, Diagnosis of Thought Prompting and Explainable Depression Detection are built on GPT-3.5/GPT-4 and Vicuna/GPT-3.5, respectively.

% \alicomment{
For the instruction fine-tuning group, \cite{hua2024large} include examples such as Mental-LLM (Alpaca/FLAN-T5 based), MentaLLaMA (LLaMA-2 based), ChatCounselo, ExTES-LLaMA (both LLaMA based), and BBMHR (BlenderBot-BST based). The exact number of parameters for these models (for both tuning-free prompting and instruction fine-tuning groups) is often undisclosed. Still, their reported sizes range from billions to tens of billions, reflecting their substantial processing power. For instance, Replika is based on GPT-3 and contains 175 billion parameters.
